EASE: Entity-Aware Contrastive Learning of Sentence Embedding

We present EASE, a novel method for learning sentence embeddings via contrastive learning between sentences and their related entities. The advantage of using entity supervision is twofold: (1) entities have been shown to be a strong indicator of text semantics and thus should provide rich training signals for sentence embeddings; (2) entities are defined independently of languages and thus offer useful cross-lingual alignment supervision. We evaluate EASE against other unsupervised models both in monolingual and multilingual settings. We show that EASE exhibits competitive or better performance in English semantic textual similarity (STS) and short text clustering (STC) tasks and it significantly outperforms baseline methods in multilingual settings on a variety of tasks. Our source code, pre-trained models, and newly constructed multilingual STC dataset are available at https://github.com/studio-ousia/ease.

==> sections/analysis/modularity.tex <==
We further analyze the effect of entity CL in terms of the language-wise distributions of embeddings.
Our intuition is that high-quality multilingual embeddings that capture language-agnostic semantics should be well mixed across languages, \ie, not forming clusters within languages.
To confirm this intuition, we evaluate multilingual sentence embeddings intrinsically by measuring the \emph{modularity} \citep{fujinuma-etal-2019-resource} of the embedding space.
% which is shown to correlate well with the quality of bilingual word embeddings.

Modularity measures the extent to which multilingual embeddings form clusters within languages.
The score is computed from the $k$-nearest neighbor graph of embeddings and we set $k=5$ in this experiment.
The maximum value of modularity is 1, which means the neighbors of every node are all in the same language, and the minimum value 0 means the embeddings are completely randomly distributed regardless of language.
Our initial hypothesis was that the EASE model exhibits lower modularity than SimCSE given the cross-lingual alignment information from entities, but as we will see below, this turns out not to hold true.

We compute the modularity scores for parallel sentences in the Tatoeba dataset for each language pair, and observe a similar trend across language pairs (comprehensive results in \Appendix{appendix:modularity}).
We present the results of mBERT-based models from the Japanese-English parallel sentences in \Figure{fig:modularity} along with the visualization of embeddings distribution with PCA.

Firstly, we observe that SimCSE and EASE exhibit reasonably lower modularity from mBERT, showing that the sentence-level training in SimCSE and EASE both mitigate the modularity of sentence embeddings.
On the other hand, LaBSE, a model trained with rich parallel corpora, exhibit the lowest modularity, indicating the gap between the effect of using parallel resources in LaBSE and weaker supervisions in SimCSE and EASE.

When comparing SimCSE and EASE, we observe slightly higher modularity scores in EASE.
This is somewhat surprising given that in EASE outperforms SimCSE in terms of parallel sentence matching (\cref{subsec:tatoeba}).
This suggests that lower modularity, \ie, embeddings from different languages are more mixed, does not necessarily transfer to semantically aligned embeddings.
Also, this shows that entity CL in EASE does not have a strong effect of matching the embedding distributions of different languages although it does pull semantically related sentences across languages closer.


\begin{figure*}[t]
\begin{minipage}{.25\linewidth}
\centering
\subfloat[mBERT: 0.66.]{\label{fig:modularity-mBERT}\includegraphics[height=3.5cm]{figures/modularity/mBERT_avg-tatoeba.jpn-eng.png}}
\end{minipage}\hfill
\begin{minipage}{.25\linewidth}
\centering
\subfloat[SimCSE: 0.48.]{\label{fig:modularity-SimCSE}\includegraphics[height=3.5cm]{figures/modularity/SimCSE-mBERT-tatoeba.jpn-eng.png}}
\end{minipage}\hfill
\begin{minipage}{.25\linewidth}
\centering
\subfloat[EASE: 0.52.]{\label{fig:modularity-EASE}\includegraphics[height=3.5cm]{figures/modularity/EASE-mBERT-tatoeba.jpn-eng.png}}
\end{minipage}\hfill
\begin{minipage}{.25\linewidth}
\centering
\subfloat[LaBSE: 0.12.]{\label{fig:modularity-LaBSE}\includegraphics[height=3.5cm]{figures/modularity/LaBSE-tatoeba.jpn-eng.png}}
\end{minipage}
\caption{The PCA visualizations and modularity scores of the en-ja sentence embeddings in the Tatoeba dataset.}
\label{fig:modularity}
\end{figure*}


==> sections/appendices/lareqa.tex <==
\section{Cross-lingual QA Retrieval}
We evaluate multilingual sentence embeddings with a cross-lingual information retrieval task, LAReQA \citep{roy-etal-2020-lareqa}.
% Why this task?
This task is designed to measure strong alignment among languages: the model is asked to retrieve answer sentences from a multilingual candidate pool.
This means that the model needs to avoid ``language bias'', where a model prefers irrelevant answers in the question's language over correct results from another language.

% \paragraph{Model}
Following \citet{roy-etal-2020-lareqa}, all the models evaluated are the dual encoder model \citep{Gillick2018EndtoEndRI}.
The questions and answers are encoded as the pooled sentence embeddings from the pretrained model, and the candidate with the highest cosine similarity is retrieved as the answer.
The model is trained with the in-batch sampled softmax loss \citep{Henderson2017EfficientNL}.
We evaluate the models in the cross-lingual transfer setting, fine-tuning the models with the English SQuAD dataset \citep{rajpurkar-etal-2016-squad} and evaluate mean average precision (mAP) \citep{roy-etal-2020-lareqa} with $k=1000$.

% \paragraph{Results}
 Table \ref{table:lareqa} summarizes the results.
The EASE models consistently outperform the baselines, indicating that the multilingual sentence embeddings is also effective in the cross-lingual retrieval task with fine-tuning.

\begin{table}
\centering
\begin{tabular}{lc}\toprule
mBERT (avg.) & 27.4\\
mBERT (cls) & 29.2\\
SimCSE-mBERT\ba & 29.8\\
EASE-mBERT\ba & 29.8\\ \midrule
XLM-R (avg.) & 34.7\\
XLM-R (cls) & 34.6\\
SimCSE-XLM-R\ba & 35.1\\
EASE-XLM-R\ba & 35.4\\
\bottomrule
\end{tabular}
\caption{The mAP scores on the LAReQA dataset.}
\label{table:lareqa}
\end{table}


==> sections/appendices/modularity.tex <==
\section{Modularity}
\label{appendix:modularity}
In \cref{subsec:modularity}, we presented the modularity scores of Japanese-English parallel sentences from the Tatoeba dataset.
Here we present the results of the all 112 languages in the dataset in \Figure{fig:modularity-all}, plotting the modularity score for each language as well as the accuracy of parallel sentence matching.

Here, we can confirm the trends discussed in \cref{subsec:modularity}: SimCSE and EASE exhibit lower modularity scores than mBERT; LaBSE shows lowest modularity scores overall; and EASE shows higher modularity scores than SimCSE but performs better on parallel sentence matching.

Within a single model, we can see a clear pattern indicating that the lower the modularity score, the higher the accuracy of parallel sentence matching with different languages.
However, the comparison between SimCSE and EASE suggests that this does not necessarily hold when comparing different models.




\begin{figure}[h]

\begin{minipage}{.25\linewidth}
\centering
\subfloat[mBERT: 0.22 / 0.64.]{\label{fig:modularity-mBERT-all}\includegraphics[height=3.5cm]{figures/modularity/mBERT_avg-all.png}}
\end{minipage}\hfill
\begin{minipage}{.25\linewidth}
\centering
\subfloat[SimCSE: 0.23 / 0.49.]{\label{fig:modularity-SimCSE-all}\includegraphics[height=3.5cm]{figures/modularity/SimCSE-mBERT-all.png}}
\end{minipage}\hfill
\begin{minipage}{.25\linewidth}
\centering
\subfloat[EASE: 0.33 / 0.53.]{\label{fig:modularity-EASE-all}\includegraphics[height=3.5cm]{figures/modularity/EASE-mBERT-all.png}}
\end{minipage}\hfill
% \vspace{-1pt}
\begin{minipage}{.25\linewidth}
\centering
\subfloat[LaBSE: 0.83 / 0.17.]{\label{fig:modularity-LaBSE-all}\includegraphics[height=3.5cm]{figures/modularity/LaBSE-all.png}}
\end{minipage}
\caption{The accuracy scores of parallel sentence matching (x-axis) and modularity scores (y-axis) for all language pairs in the Tatoeba dataset. The values in the caption denotes (the average accuracy / the average modularity).}
\label{fig:modularity-all}
\end{figure}


==> sections/appendices/monolingual_batch.tex <==
\begin{table}
\centering
\begin{tabular}{lccc}
Model & mBERT & XLM-R \\ \hline
SimCSE (random) & 50.9 & 54.1 \\
SimCSE (mono) & 54.2 & 52.7 \\ \hline
EASE (random) & 57.2 & 57.1 \\
EASE (mono) & 53.7 & 54.2\\ \hline
\end{tabular}
\caption{mSTS}
\label{table: mono_batch}
\end{table}
